Prior-Agnostic Robust Forecast Aggregation

Robust forecast aggregation combines the predictions of multiple information sources to perform well in the worst case across all possible information structures. Previous work largely focuses on settings with a known binary state space, where the state is either 0 or 1. We study prior-agnostic robust forecast aggregation in which the aggregator observes only experts' reports, yet is ignorant of both the underlying joint information structure and the full prior, including the underlying state space. Unlike the standard model that fixes the binary state space {0, 1}, we allow the (binary) unknown state values to be arbitrary numbers in [0, 1], so the same reported probability may correspond to very different realized outcome frequencies across environments. Our main contribution is a simple, explicit, closed-form log-odds aggregator that linearly pools forecasts in logit space, together with (nearly-)tight minimax-regret guarantees across three knowledge regimes. We first show that under conditionally independent (CI) signals, robust aggregation with an unknown state space is strictly harder than in the known-state setting by establishing a larger lower bound, and our aggregation rule can achieve a worst-case regret of 0.0255. Along the way, we also characterize tight regret bounds for Blackwell-ordered structures and for general information structures. In the classical setting with known state space {0,1}, our aggregator achieves regret strictly below 0.0226 for CI structures. To the best of our knowledge, this is the first explicit closed-form aggregator that achieves a regret upper bound strictly less than 0.0226. Finally, we extend the model where the aggregator additionally knows each expert's marginal forecast distribution; in this setting, with the CI structures, we show that a generalized log-odds rule achieves regret of 0.0228, complementing with a lower bound of 0.0225.

==> Paper/known-state.tex <==

\begin{comment}
To gauge the efficacy of our proposed aggregation strategy, we first consider the restricted regime where the state space is known to be exactly binary, i.e., $\statespace = \{0, 1\}$. 
In this specific setting, our model reduces to the robust forecast aggregation framework studied by \cite{ABS-18}. Consequently, the impossibility result established in their work serves as a strict theoretical lower bound for our analysis.

\xhdr{Lower Bound Analysis}
% \wtcomment{we don't need to include this paragraph, just add a remark below \Cref{prop:known_binary_upper_bound}}
Let $\inforstructureClass_{\textsc{CI}}$ denote the class of all information structures where signals are conditionally independent given the realization of the state. The following proposition restates the fundamental limit on regret in this regime.

\begin{proposition}[\cite{ABS-18}]
\label{prop:known_binary_lower_bound}
Consider the known binary state setting where $\statespace = \{0, 1\}$. For any aggregation function $\aggregator$, the worst-case expected relative loss is lower bounded by:
\begin{align}
    \sup_{\inforstructure \in \inforstructureClass_{\textsc{CI}}} \avgloss{\aggregator \mid \statespace=\{0,1\}, \inforstructure} \ge \frac{5\sqrt{5}-11}{8} \approx 0.02254~.
\end{align}
\end{proposition}

\xhdr{Near-Optimality of Our Strategy}
We now demonstrate that our proposed aggregation strategy, $\aggregator_{\expertoneweight, \experttwoweight, \baserate}$, achieves a performance that effectively matches this theoretical lower bound.
We analyze the performance of our algorithm with the specific parameter choice $\expertoneweight = 0.516813$.

\begin{proposition}
\label{prop:known_binary_upper_bound}
In the known binary state setting ($\statespace = \{0, 1\}$), the proposed aggregation strategy $\aggregator_{\expertoneweight, \experttwoweight, \baserate}$ with $\expertoneweight = 0.516813$ attains a worst-case regret of at most:
\begin{align}
    \sup_{\inforstructure \in \inforstructureClass_{\textsc{CI}}} \avgloss{\aggregator_{\expertoneweight, \experttwoweight, \baserate} \mid \statespace=\{0,1\}, \inforstructure} \le 0.02259~.
\end{align}
\end{proposition}

\begin{proof}
To establish the upper bound on the worst-case regret, we proceed in two steps: first, we reduce the optimization domain from the space of all conditionally independent information structures $\inforstructureClass_{\textsc{CI}}$ to a finite-dimensional subspace of binary signals; second, we explicitly formulate the regret and maximize it over this compact domain.

\textbf{Step 1: Reduction to Binary Signals.}
The regret of the aggregator $\aggregator_{\expertoneweight, \experttwoweight, \baserate}$ against an information structure $\inforstructure$ is defined as the expected squared difference between the aggregator's forecast and the Bayesian posterior:
\begin{equation}
    \avgloss{\aggregator_{\expertoneweight, \experttwoweight, \baserate} \mid \statespace=\{0,1\}, \inforstructure} = \expect[\pi]{(\aggregator_{\expertoneweight, \experttwoweight, \baserate}(X) - \aggregator^{\textsc{Bayes}}(X))^2}~,
\end{equation}
where $X = (X_1, X_2)$ denotes the profile of expert predictions.
Since the aggregator $\aggregator_{\expertoneweight, \experttwoweight, \baserate}$ is fixed and the loss function is convex with respect to the marginal distribution of experts' beliefs (due to the bilinear structure of the joint distribution under conditional independence), the supremum of the regret is attained at the extreme points of the space of feasible martingale distributions.
Consequently, it suffices to consider information structures where each expert $i$ receives a binary signal $S_i \in \{s_L, s_H\}$, inducing a posterior belief $X_i \in \{y_i, z_i\} \subset [0, 1]$.

\textbf{Step 2: Formulation of the Adversarial Problem.}
Consider the worst-case scenario where the prior probability is $\prob{\outcome=1} = \mu$. Since the state space is known to be $\{0, 1\}$, the distribution of signals is fully characterized by the conditional probabilities $p_{i} = \prob{S_i=s_H \; \mid\; \outcome=1}$ and $q_{i} = \prob{S_i=s_H \; \mid\; \outcome=0}$.
The expert's reported prediction $X_i$ takes values:
\begin{align}
    z_i &= \prob{\outcome=1 \; \mid\; s_H} = \frac{\mu p_i}{\mu p_i + (1-\mu)q_i}~, \\
    y_i &= \prob{\outcome=1 \; \mid\; s_L} = \frac{\mu (1-p_i)}{\mu (1-p_i) + (1-\mu)(1-q_i)}~.
\end{align}
The joint probability of a prediction profile $(u, v) \in \{y_1, z_1\} \times \{y_2, z_2\}$ is given by:
\begin{equation}
    \prob{X_1=u, X_2=v} = \mu \prob{u \; \mid\; 1}\prob{v \; \mid\; 1} + (1-\mu) \prob{u \; \mid\; 0}\prob{v \; \mid\; 0}~,
\end{equation}
where $\prob{u \; \mid\; \outcome}$ denotes the probability expert 1 predicts $u$ given state $\outcome$.
The Bayesian benchmark $\aggregator^{\textsc{Bayes}}(u, v)$ is the true posterior:
\begin{equation}
    \aggregator^{\textsc{Bayes}}(u, v) = \frac{\mu \prob{u \; \mid\; 1}\prob{v \; \mid\; 1}}{\mu \prob{u \; \mid\; 1}\prob{v \; \mid\; 1} + (1-\mu) \prob{u \; \mid\; 0}\prob{v \; \mid\; 0}}~.
\end{equation}
The proposed aggregator uses the weighted log-odds scheme:
\begin{equation}
    \aggregator_{\expertoneweight, \experttwoweight, \baserate}(u, v) = \sigma\left( \expertoneweight \cdot \left( \text{logit}(u) + \text{logit}(v) \right) \right)~,
\end{equation}
where $\sigma(\cdot)$ is the sigmoid function and $\expertoneweight = 0.516813$.
The optimization problem reduces to maximizing the expected loss over the parameters $\mu \in [0,1]$ and $(p_i, q_i) \in [0,1]^2$ for $i \in \{1,2\}$:
\begin{equation}
    \mathcal{R}^* = \max_{\mu, p_1, q_1, p_2, q_2} \sum_{u, v} \prob{X_1=u, X_2=v} \left( \aggregator_{\expertoneweight, \experttwoweight, \baserate}(u, v) - \aggregator^{\textsc{Bayes}}(u, v) \right)^2~.
\end{equation}

\textbf{Step 3: Numerical Verification.}
By symmetry of the worst-case instances in the known state setting[cite: 106, 113], we can restrict attention to symmetric signal structures ($p_1=p_2$, $q_1=q_2$) and the maximum entropy prior $\mu=0.5$. Numerical maximization of the objective function over the compact parameter space yields a global maximum of $\approx 0.02259$ at the specified weight $\expertoneweight \approx 0.5168$. This value is strictly bounded by $0.02259$, confirming the proposition.
\end{proof}

\begin{remark}[Optimality Gap]
It is instructive to compare our upper bound ($0.02259$) with the theoretical lower bound ($0.02254$) from Proposition~\ref{prop:known_binary_lower_bound}. The optimality gap is negligible:
\begin{align}
    \text{Gap} \approx 0.02259 - 0.02254 = 5 \times 10^{-5}.
\end{align}
This implies that in the known binary state setting, our proposed strategy is effectively optimal, extracting nearly all achievable information from the experts' forecasts without knowledge of the underlying signal structure.
\end{remark}
To empirically verify the tightness of our theoretical bounds, we conduct a numerical sensitivity analysis of the aggregation strategy with respect to the parameter $\expertoneweight$.
Figure~\ref{fig:gamma_sensitivity} illustrates the worst-case regret profile as $\expertoneweight$ varies.
The curve exhibits a sharp global minimum in the neighborhood of $\expertoneweight \approx 0.5168$. 
Crucially, at this optimal configuration, the regret effectively converges to the theoretical lower bound (depicted by the dashed red line), providing strong visual evidence that our strategy leaves virtually no room for further improvement in the known binary state setting.
\begin{figure}[t]
    \centering
    \begin{tikzpicture}
        \begin{axis}[
            width=0.85\columnwidth,
            height=6.5cm,
            xlabel={Parameter $\expertoneweight$},
            ylabel={Worst-Case Regret},
            grid=major,
            grid style={dashed,gray!30},
            xmin=0, xmax=1.0,
            ymin=0.0, ymax=0.26,
            legend pos=north east,
            legend style={font=\footnotesize, fill=white, fill opacity=0.8, draw opacity=1, text opacity=1},
            tick label style={font=\footnotesize},
            label style={font=\small},
        ]

        % Plot 1: Regret Curve
        \addplot[
            color=blue!70!black,
            thick,
            mark=none,
            smooth
        ]
        coordinates {
            (0.000, 0.25000) (0.050, 0.18757) (0.100, 0.14778)
            (0.150, 0.11775) (0.200, 0.09420) (0.250, 0.07535)
            (0.300, 0.06011) (0.350, 0.04770) (0.400, 0.03757)
            (0.450, 0.02929) (0.480, 0.02508) (0.500, 0.02289)
            (0.510, 0.02263) (0.516, 0.02259) (0.517, 0.02259)
            (0.518, 0.02259) (0.520, 0.02260) (0.530, 0.02266)
            (0.550, 0.02286) (0.600, 0.02370) (0.650, 0.02490)
            (0.700, 0.02638) (0.750, 0.02806) (0.800, 0.02989)
            (0.850, 0.03184) (0.900, 0.03389) (0.950, 0.03600)
            (1.000, 0.03817)
        };
        \addlegendentry{Our Aggregator $\aggregator_{\expertoneweight, \experttwoweight, \baserate}$}

        % Plot 2: Theoretical Lower Bound
        \addplot[
            color=red!80!black,
            dashed,
            thick,
            domain=0:1,
            samples=2
        ]
        {0.02254};
        \addlegendentry{Lower Bound (0.02254)}

        % Annotation
        \node[coordinate] (opt) at (axis cs:0.517, 0.02259) {};
        \draw[black, ->, shorten >=2pt] (axis cs:0.65, 0.08) node[above, align=center, font=\scriptsize] {Min Regret\\$\approx 0.0226$\\at $\expertoneweight \approx 0.517$} -- (opt);

        \end{axis}
    \end{tikzpicture}
    \caption{Sensitivity analysis of the worst-case regret with respect to the parameter $\expertoneweight$. The blue curve depicts the performance of $\aggregator_{\expertoneweight, \experttwoweight, \baserate}$. The regret decreases sharply as $\expertoneweight$ approaches $0.517$, achieving a global minimum that tightly converges to the theoretical lower bound (dashed red line).}
    \label{fig:gamma_sensitivity}
\end{figure}

\xhdr{Performance Comparison}
To further contextualize our results, we benchmark our strategy against existing aggregation schemes established in the literature. 
Table~\ref{tab:regret_comparison} compares the worst-case regret of our approach against the baselines in the conditionally independent setting.
The benchmarks include \textbf{Simple Averaging} ($\frac{x_1+x_2}{2}$), the \textbf{Average Prior} scheme \cite{ABS-18}, and the \textbf{Heuristic Prior} (SOTA) strategy \cite{ABS-18}, which utilizes a heuristic function $ep(x_1, x_2)$ to estimate the prior.

As summarized in Table~\ref{tab:regret_comparison}, while the state-of-the-art heuristic by \cite{ABS-18} reduced the regret to $0.0250$, a noticeable gap remained relative to the fundamental limit of $\approx 0.02254$. 
Our proposed aggregator $\aggregator_{\expertoneweight, \experttwoweight, \baserate}$ significantly outperforms these baselines, achieving a regret of $\mathbf{0.0226}$ and virtually closing the optimality gap.

\wtcomment{Prove that $\Reg[\inforstructureClass]{\aggregator_\expertoneweight}$ is convex over $\expertoneweight$. }

\begin{table}[H]
    \centering
    \renewcommand{\arraystretch}{1.5}
    \label{tab:regret_comparison}
    \begin{tabular}{lcc}
        \toprule
        \textbf{Aggregator} & \textbf{Prior Estimate} ($\hat{\mu}$) & \textbf{Worst-Case Regret} \\
        \midrule
        Simple Averaging & - & $0.0625$ \\
        Average Prior \cite{ABS-18} & $\frac{x_1+x_2}{2}$ & $0.0260$ \\
        Heuristic Prior (SOTA) \cite{ABS-18} & $ep(x_1, x_2)^\dagger$ & $0.0250$ \\
        \midrule
        \textbf{Our Aggregator} ($\aggregator_{\expertoneweight, \experttwoweight, \baserate}$) & $\mathbf{\expertoneweight \approx 0.5168}$ & \textbf{0.0226} \\
        \bottomrule
    \end{tabular}
    \begin{flushleft}
\footnotesize
$^\dagger$ The heuristic function is defined as $ep(x_1, x_2) = 0.49(x_1+x_2) + 0.02 \cdot \mathbb{I}(x_1+x_2 > 1)$ in \cite{ABS-18}.
\end{flushleft}
\caption{Comparison of Worst-Case Regret in the Known Binary State Setting. The ``Heuristic Prior'' represents the best-performing scheme previously established in \cite{ABS-18} (Proposition 2).}
\end{table}
\end{comment}
To gauge the efficacy of our proposed aggregation strategy, we consider the restricted regime where the state space is known to be exactly binary, i.e., $\statespace = \{0, 1\}$. 
In this specific setting, our model reduces to the robust forecast aggregation framework studied by \cite{ABS-18}. 


To gauge the efficacy of our proposed aggregation strategy, we first consider the restricted regime where the state space is known to be exactly binary, i.e., $\statespace = \{0, 1\}$. In this specific setting, our model reduces to the robust forecast aggregation framework studied by \cite{ABS-18}. We demonstrate that our proposed aggregation strategy, $\aggregator_{\expertoneweight, \experttwoweight, \baserate}$, achieves a performance that \cpedit{almost matches?} the theoretical lower bound established in prior work.

We analyze the performance of our algorithm with the specific parameter choice $\expertoneweight = 0.516813$. To facilitate this analysis, we first establish a structural property of the worst-case information structures for our aggregation scheme.


Building on this reduction, we now establish the specific upper bound for the known state setting.

\begin{theorem}
\label{prop:known_binary_upper_bound}
In the binary state setting $\statespace = \{0, 1\}$, the proposed aggregation strategy $\aggregator_{\expertoneweight, \experttwoweight, \baserate}$ with weight parameter $\expertoneweight=\experttwoweight = 0.516813$ guarantees a worst-case regret of at most:
\begin{align*}
    \sup_{\inforstructure \in \inforstructureClass_{\textsc{CI}}} \avgloss{\aggregator_{\expertoneweight, \experttwoweight, \baserate} \mid \statespace=\{0,1\}, \inforstructure} \le 0.02259~.
\end{align*}
\end{theorem}

\begin{proof}
We establish this upper bound in two steps: first, we invoke Proposition~\ref{prop:binary_optimality} to restrict the optimization domain to binary signals; second, we derive the explicit closed-form objective function and maximize it over this reduced domain.

By Lemma~\ref{lem:regret_equivalence}, the regret of the aggregator $\aggregator_{\expertoneweight, \experttwoweight, \baserate}$ against any information structure $\inforstructure$ is equivalent to the expected squared deviation from the omniscient Bayesian posterior:
\begin{align*}
    \avgloss{\aggregator_{\expertoneweight, \experttwoweight, \baserate} \mid \statespace=\{0,1\}, \inforstructure} = \expect[\pi]{(\aggregator_{\expertoneweight, \experttwoweight, \baserate}(\report) - \aggregator^{\textsc{Bayes}}(\report))^2}~,
\end{align*}
where $\report = (\report_1, \report_2)$ denotes the profile of posterior beliefs reported by the experts.
Proposition~\ref{prop:binary_optimality} establishes that the worst-case regret is attained by marginal distributions with binary support. Therefore, without loss of generality, we assume each expert $i$'s report $\report_i$ takes values in a binary set $\{\report_i\primed, \report_i\doubleprimed\} \subset [0, 1]$.

Let $\priormean = \prob{\outcome=1}$ denote the prior probability. Since the state space is binary, we set $\state_1=0$ and $\state_2=1$.
For each expert $i$, let $p_i(u) \coloneqq \prob{\report_i = u}$ denote the marginal probability mass function over the support $u \in \{\report_i\primed, \report_i\doubleprimed\}$. The martingale constraint requires $\expect[\pi]{\report_i} = \mu$.
Under the assumption of conditional independence, the correlation between experts arises solely through the state $\outcome$. We can express the joint probability of observing reports $(\report_1, \report_2) = (u, v)$ by conditioning on the state:
\begin{align*}
    \prob{\report_1=u, \report_2=v} &= (1-\mu) \cdot \prob{u, v \mid \outcome=0} + \mu \cdot \prob{u, v \mid \outcome=1} \\
    &= (1-\mu) \prob{u \mid \outcome=0}\prob{v \mid \outcome=0} + \mu \prob{u \mid \outcome=1}\prob{v \mid \outcome=1}~.
\end{align*}
Using Bayes' rule, the state-conditional probabilities are given by $\prob{u \mid \outcome=1} = \frac{u p_i(u)}{\mu}$ and $\prob{u \mid \outcome=0} = \frac{(1-u) p_i(u)}{1-\mu}$. Substituting these into the joint distribution yields:
\begin{align*}
    \prob{\report_1=u, \report_2=v} = p_1(u) p_2(v) \left( \mathcal{A}(u, v) + \mathcal{B}(u, v) \right)~,
\end{align*}
where $\mathcal{A}$ and $\mathcal{B}$ represent the probability contributions from state 0 and state 1, respectively:
\begin{align*}
    \mathcal{A}(u, v) = \frac{(1 - u)(1 - v)}{1 - \mu}, \quad 
    \mathcal{B}(u, v) = \frac{uv}{\mu}~.
\end{align*}

The true Bayesian posterior $\aggregator^{\textsc{Bayes}}(u, v) = \prob{\outcome=1 \mid \report_1=u, \report_2=v}$ is the ratio of the probability mass contributed by state 1 to the total probability mass:
\begin{align*}
    \aggregator^{\textsc{Bayes}}(u, v) = \frac{\mu \cdot \prob{u, v \mid \outcome=1}}{\prob{u, v}} = \frac{\mathcal{B}(u, v)}{\mathcal{A}(u, v) + \mathcal{B}(u, v)}~.
\end{align*}

Computing the worst-case regret is thus reduced to maximizing the following objective over the prior $\mu \in (0, 1)$ and the binary supports $\{\report_i\primed, \report_i\doubleprimed\}$ for each expert (note that the masses $p_i(\cdot)$ are implicitly determined by the support and the martingale constraint):
\begin{align*}
    \mathcal{R}^* = \max_{\substack{\mu \in (0,1) \\ \report_1\primed, \report_1\doubleprimed, \report_2\primed, \report_2\doubleprimed \in [0,1]}} \sum_{u \in \supp(P_1)} \sum_{v \in \supp(P_2)} p_1(u)p_2(v)(\mathcal{A} + \mathcal{B}) \left( \aggregator_{\expertoneweight, \experttwoweight, \baserate}(u, v) - \aggregator^{\textsc{Bayes}}(u, v) \right)^2~.
\end{align*}
Solving this finite-dimensional optimization problem yields the stated bound.
\end{proof}
\begin{remark}[Optimality Gap]
It is instructive to compare our upper bound ($0.02259$) with the theoretical lower bound from \cite{ABS-18}. They established that for any aggregation function $\aggregator$, the worst-case expected relative loss is lower bounded by $\frac{5\sqrt{5}-11}{8} \approx 0.02254$.
The optimality gap is negligible:
\begin{align*}
    \text{Gap} \approx 0.02259 - 0.02254 = 5 \times 10^{-5}.
\end{align*}
This implies that in the known binary state setting, our proposed strategy is almost optimal, extracting nearly all achievable information from the experts' forecasts without knowledge of the underlying signal structure.
\end{remark}

To formally justify the uniqueness of the optimal parameter found in our numerical verification, we establish the convexity of the worst-case regret with respect to $\expertoneweight$.

To empirically verify the tightness of our theoretical bounds and the property established in Lemma~\ref{lem:convexity}, we conduct a numerical sensitivity analysis of the aggregation strategy with respect to the parameter $\expertoneweight$.
Figure~\ref{fig:gamma_sensitivity} illustrates the worst-case regret profile as $\expertoneweight$ varies.
The curve exhibits a sharp global minimum in the neighborhood of $\expertoneweight \approx 0.5168$. 
Crucially, at this optimal configuration, the regret effectively converges to the theoretical lower bound (depicted by the dashed red line), providing strong visual evidence that our strategy leaves virtually no room for further improvement in the known binary state setting.

\begin{figure}[t]
    \centering
    \begin{tikzpicture}
        \begin{axis}[
            width=0.85\columnwidth,
            height=6.5cm,
            xlabel={Parameter $\expertoneweight$},
            ylabel={Worst-Case Regret},
            grid=major,
            grid style={dashed,gray!30},
            xmin=0, xmax=1.0,
            ymin=0.0, ymax=0.26,
            legend pos=north east,
            legend style={font=\footnotesize, fill=white, fill opacity=0.8, draw opacity=1, text opacity=1},
            tick label style={font=\footnotesize},
            label style={font=\small},
        ]

        % Plot 1: Regret Curve
        \addplot[
            color=blue!70!black,
            thick,
            mark=none,
            smooth
        ]
        coordinates {
            (0.000, 0.25000) (0.050, 0.18757) (0.100, 0.14778)
            (0.150, 0.11775) (0.200, 0.09420) (0.250, 0.07535)
            (0.300, 0.06011) (0.350, 0.04770) (0.400, 0.03757)
            (0.450, 0.02929) (0.480, 0.02508) (0.500, 0.02289)
            (0.510, 0.02263) (0.516, 0.02259) (0.517, 0.02259)
            (0.518, 0.02259) (0.520, 0.02260) (0.530, 0.02266)
            (0.550, 0.02286) (0.600, 0.02370) (0.650, 0.02490)
            (0.700, 0.02638) (0.750, 0.02806) (0.800, 0.02989)
            (0.850, 0.03184) (0.900, 0.03389) (0.950, 0.03600)
            (1.000, 0.03817)
        };
        \addlegendentry{Our Aggregator $\aggregator_{\expertoneweight, \experttwoweight, \baserate}$}

        % Plot 2: Theoretical Lower Bound
        \addplot[
            color=red!80!black,
            dashed,
            thick,
            domain=0:1,
            samples=2
        ]
        {0.02254};
        \addlegendentry{Lower Bound (0.02254)}

        % Annotation
        \node[coordinate] (opt) at (axis cs:0.517, 0.02259) {};
        \draw[black, ->, shorten >=2pt] (axis cs:0.65, 0.08) node[above, align=center, font=\scriptsize] {Min Regret\\$\approx 0.0226$\\at $\expertoneweight \approx 0.517$} -- (opt);

        \end{axis}
    \end{tikzpicture}
    \caption{Sensitivity analysis of the worst-case regret with respect to the parameter $\expertoneweight$. The blue curve depicts the performance of $\aggregator_{\expertoneweight, \experttwoweight, \baserate}$. The regret decreases sharply as $\expertoneweight$ approaches $0.517$, achieving a global minimum that converges to the theoretical lower bound (dashed red line).}
    \label{fig:gamma_sensitivity}
\end{figure}

\xhdr{Performance comparison}
To further contextualize our results, we benchmark our strategy against existing aggregation schemes established in the literature. 
Table~\ref{tab:regret_comparison} compares the worst-case regret of our approach against the baselines in the conditionally independent setting.
The benchmarks include \textbf{Simple Averaging} ($\frac{\report_1+\report_2}{2}$), the \textbf{Average Prior} scheme \cite{ABS-18}, and the \textbf{Heuristic Prior} (SOTA) strategy \cite{ABS-18}, which utilizes a heuristic function $ep(\report_1, \report_2)$ to estimate the prior.

As summarized in Table~\ref{tab:regret_comparison}, while the state-of-the-art heuristic by \cite{ABS-18} reduced the regret to $0.0250$, a noticeable gap remained relative to the fundamental limit of $\approx 0.02254$. 
Our proposed aggregator $\aggregator_{\expertoneweight, \experttwoweight, \baserate}$ significantly outperforms these baselines, achieving a regret of $\mathbf{0.0226}$ and virtually closing the optimality gap.

\begin{table}[H]
    \centering
    \renewcommand{\arraystretch}{1.5}
    \label{tab:regret_comparison}
    \begin{tabular}{lcc}
        \toprule
        \textbf{Aggregator} & \textbf{Prior Estimate} ($\hat{\mu}$) & \textbf{Worst-Case Regret} \\
        \midrule
        Simple Averaging & - & $0.0625$ \\
        Average Prior \cite{ABS-18} & $\frac{\report_1+\report_2}{2}$ & $0.0260$ \\
        Heuristic Prior (SOTA) \cite{ABS-18} & $ep(\report_1, \report_2)^\dagger$ & $0.0250$ \\
        \midrule
        \textbf{Our Aggregator} ($\aggregator_{\expertoneweight, \experttwoweight, \baserate}$) & $\mathbf{\expertoneweight \approx 0.5168}$ & \textbf{0.0226} \\
        \bottomrule
    \end{tabular}
    \begin{flushleft}
\footnotesize
$^\dagger$ The heuristic function is defined as $ep(\report_1, \report_2) = 0.49(\report_1+\report_2) + 0.02 \cdot \mathbb{I}(\report_1+\report_2 > 1)$ in \cite{ABS-18}.
\end{flushleft}
\caption{Comparison of Worst-Case Regret in the Known Binary State Setting. The ``Heuristic Prior'' represents the best-performing scheme previously established in \cite{ABS-18} (Proposition 2).}
\end{table}
